RT-Counter: Real-Time Text-Guided Open-Vocabulary Object Counting

Text-guided open-vocabulary object counting (TOOC) aims to count objects belonging to the categories specified by natural language descriptions. Although vision-language pre-trained models have been successful applied to TOOC tasks, they still struggle with fine-grained spatial understanding and real-time inference requirements in counting scenarios. To address these limitations, this paper proposes a real-time TOOC framework, called the Real-Time Counter (RT-Counter), that achieves not only good counting accuracy but also high computational efficiency. RT-Counter designs a novel Visual Prototype Textualization (VPT) module that can project learned visual features into a text feature space and then generate features containing the abstract information that is hard to capture with visual prototypes and the detailed prototype information that is difficult to describe in text, enhancing the object-level visual-language model's counting capabilities. Additionally, RT-Counter incorporates our Weaving Transformer (Weaformer) layers, maintaining high descriptive power at a fraction of the computational cost. The Weaformer layer adopts a novel hybrid attention mechanism that can efficiently weave together local and global visual features. Extensive experiments on three public datasets show that RT-Counter successfully breaks the accuracy-speed trade-off in TOOC. While achieving a competitive MAE of 13.30 on FSC147, RT-Counter operates at 112.48 FPS, making it 7.4x faster and over 4$\times$ more parameter-efficient than the existing leading methods in TOOC. Our work aims at balancing high accuracy and real-time performance in TOOC. Code is available at: https://github.com/Jason-Mar1/RT-Counter.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/4_1exp.tex <==
\section{Experiments}

\subsection{Experimental Setup}
\textbf{Hardware Environment:} All experiments are conducted on a workstation equipped with an NVIDIA RTX 3090 GPU and an AMD EPYC 7601 CPU, providing sufficient computational resources for training and evaluation.

\textbf{Software Environment:} We implement our RT-Counter framework using PyTorch 2.0 with CUDA 11.8 support for GPU acceleration and optimized tensor operations.

\textbf{Training Strategy:} We employ the AdamW optimizer with a learning rate of $1 \times 10^{-4}$ and a batch size of 8. The model is trained end-to-end without additional regularization techniques to maintain simplicity and efficiency of the training.

\textbf{Data Augmentation:} To enhance model robustness and generalization capability, we apply a comprehensive set of data augmentation techniques including random cropping, horizontal/vertical flipping, color jittering, and mosaic augmentation during training.


\textbf{Datasets:} We evaluate RT-Counter on three widely-used counting benchmarks. \textbf{FSC147} \cite{FamNet} is a few-shot counting benchmark containing 3,659 images across 147 object categories, designed to evaluate generalization to novel object classes with limited examples or zero example. \textbf{CARPK} \cite{} is a specialized dataset comprising 1,448 parking lot images focused on vehicle counting tasks, providing domain-specific evaluation for transportation scenarios. \textbf{REC-8K} \cite{rec} is a large-scale dataset with 8,000 images covering diverse scenes and object types, offering comprehensive evaluation across various counting scenarios.

\textbf{Evaluation Metrics:} We adopt standard evaluation metrics for comprehensive performance assessment. \textbf{MAE (Mean Absolute Error)} measures the average absolute difference between predicted and ground truth counts, indicating counting accuracy. \textbf{RMSE (Root Mean Square Error)} provides a measure of prediction variance and penalizes larger errors more heavily. \textbf{FPS (Frames Per Second)} evaluates real-time inference speed for practical deployment scenarios. \textbf{FLOPs} quantifies computational complexity in terms of floating-point operations. \textbf{Params} reports the total number of model parameters, indicating model size.


\subsection{Comparison with SOTA Methods}
\paragraph{Results on FSC147:}
Table~\ref{tab:counting_methods} presents performance comparisons on the FSC147 dataset. Our RT-Counter achieves the best results among differentiable text-based methods with MAE of 13.37 and RMSE of 95.99 on the test set. %Text-based methods generally outperform visual prototype-based approaches, demonstrating the importance of semantic understanding in few-shot counting. 
Among visual prototype methods, DAVE performs best (MAE: 15.14), while traditional methods like FamNet show significantly higher errors.

Our method achieves a 17.9\% improvement over the previous best differentiable text-based method (CounTX, MAE: 16.28) while maintaining end-to-end trainability. Notably, our approach approaches the performance of non-differentiable methods like CountGD (MAE: 12.98) while offering the advantages of gradient-based optimization. The results validate that our Visual Prototype Textualization module successfully bridges visual and textual information, enabling superior counting accuracy compared to existing differentiable approaches across diverse object categories.\par
\paragraph{Results on Rec-8K:}










\begin{table}[t]
\centering
\caption{Performance Comparison on Rec-8K.}
\label{tab:8k_perfor}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Val Set}} & \multicolumn{2}{c}{\textbf{Test Set}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \textbf{MAE $\downarrow$} & \textbf{RMSE $\downarrow$} & \textbf{MAE $\downarrow$} & \textbf{RMSE $\downarrow$} \\
\midrule
Mean & 14.28 & 27.75 & 13.75 & 25.91 \\
ZSC$^{ResNet_{50}}$ & 14.84 & 31.30 & 14.93 & 29.72 \\
ZSC$^{SwinT}$ & 12.96 & 26.74 & 13.00 & 29.07 \\
CounTX & 11.88 & 27.04 & 11.84 & 25.62 \\
GroundingDINO$^{SwinT}$ & 9.03 & 21.98 & 8.88 & 21.95 \\
GroundingREC$^{SwinT}$ & 6.80 & 18.13 & 6.50 & 19.79 \\
CAD-GD$^{SwinT}$ & 5.43 & 15.01 & 5.29 & 17.08 \\
% \textbf{CAD-GD$^\dagger$ (ours)} (Swin-T) & \textbf{4.58} & \textbf{13.24} & \textbf{4.59} & \textbf{14.68} \\
GroundingREC$^{SwinB}$ & 5.66 & 15.24 & 5.42 & 18.47 \\
% CAD-GD$^{SwinB}$ & \textbf{4.83} & \textbf{13.52} & \textbf{4.94} & \textbf{14.65} \\
CAD-GD$^{SwinB}$ & \textbf{4.23} & \textbf{13.14} & \textbf{4.34} & \textbf{12.93} \\ \hline
ours & & & & \\
\bottomrule
\end{tabular}%
}
\end{table}




\begin{table}[htbp]
\centering
\caption{Performance Comparison on CARPK Dataset}
\label{tab:carpk_text_methods}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Dataset} & \textbf{Method} & \textbf{MAE $\downarrow$} & \textbf{RMSE $\downarrow$} \\
\midrule
\multirow{4}{*}{CARPK} 
& CLIP-count   & 11.96 & 16.61 \\
& CounTX & 6.13 & 10.87 \\
& VLCounter  & 6.46 & 8.68 \\
& CountGD   & \textbf{3.83} & \textbf{5.41} \\ \hline
& Ours & & \\
\bottomrule
\end{tabular}
\end{table}


\paragraph{Results on CARPK:}



\begin{table}[htbp]
\centering
\caption{Model Efficiency Comparison}
\label{tab:efficiency_comparison}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Method} & \textbf{Parameters $\downarrow$} & \textbf{FPS $\uparrow$} & \textbf{FLOPs $\downarrow$} \\
\midrule
CountGD & 236M & 4.93 & 259.87G \\
% YOLO-Count & 68M & 50.41 & -- \\
CLIP-Count & 149M & 10.34 & 123.06G \\
CounTX & 161M & 9.98 & 83.88G \\
DAVE & 150M & 2.37 & 170.77G \\
\textbf{Ours} & \textbf{28M} & \textbf{187.2} & \textbf{21.37G} \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Model Efficiency Comparison. Runtime Analysis.}


\begin{table}[htbp]
\centering
\caption{Ablation Study Results on FSC147.}
\label{tab:ablation_study}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{FSC147 Test}} \\
\cmidrule(lr){2-3}
& \textbf{MAE} & \textbf{RMSE} \\
\midrule
Baseline (zero-shot) & 33.28 & 122.87 \\
Baseline (Point) & 30.55 & 109.08 \\
w/o FE & 22.98 & 108.32 \\
w/o VPT & 16.09 & 100.84 \\
\textbf{Ours} & \textbf{13.37} & \textbf{95.99} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\caption{Comparison of VPT Integration on FSC147 Performance.}
\label{tab:vpt_comparison}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Test Set}} \\
\cmidrule(lr){2-3}
& \textbf{MAE} & \textbf{RMSE} \\
\midrule
CounTX & 16.28 & 106.41 \\
CounTX + VPT & 15.39 & 105.81 \\
Ours w/o VPT & 16.09 & 100.84 \\
\textbf{Ours} & \textbf{13.37} & \textbf{95.99} \\
\bottomrule
\end{tabular}
\end{table}
\subsection{Ablation Studies}

% \subsection{Runtime Analysis}
